Plan-Structured Deep Neural Network Models for Query Performance Prediction

Query performance prediction, the task of predicting the latency of a query, is one of the most challenging problem in database management systems. Existing approaches rely on features and performance models engineered by human experts, but often fail to capture the complex interactions between query operators and input relations, and generally do not adapt naturally to workload characteristics and patterns in query execution plans. In this paper, we argue that deep learning can be applied to the query performance prediction problem, and we introduce a novel neural network architecture for the task: a plan-structured neural network. Our approach eliminates the need for human-crafted feature selection and automatically discovers complex performance models both at the operator and query plan level. Our novel neural network architecture can match the structure of any optimizer-selected query execution plan and predict its latency with high accuracy. We also propose a number of optimizations that reduce training overhead without sacrificing effectiveness. We evaluated our techniques on various workloads and we demonstrate that our plan-structured neural network can outperform the state-of-the-art in query performance prediction.

==> neural_arch__Ryan_Marcus_s_conflicted_copy_2018-09-26_.tex <==
\section{Neural architecture}\label{sec:arch}
\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figures/general_arch-crop.pdf}
\caption{\small Each node in a query execution plan is mapped to a neural unit corrosponding to the relational operator.}
\label{fig:nn_general}
\end{figure}

In this section, the proposed novel neural architecture for query performance prediction is described. The architecture is depicted in Figure~\ref{fig:nn_general}. At a high level, our architecture works by constructing a unique \emph{neural unit}, a small neural network, for each type of relational operator used by a DBMS' execution engine. When estimating the latency of a given query execution plan, these neural units are then connected in a tree structure, matching the shape of a  query's execution plan. Section~\ref{sec:units} discusses how each individual neural unit is constructed, and Section~\ref{sec:tree} explains how the neural units are combined into tree structures.

\subsection{Operator-level neural units}
\label{sec:units}
Our proposed new architecture will model each operator of a DBMS' execution engine with a unique corresponding neural unit, responsible for learning the performance of that particular operator, e.g.~a unique neural unit for joins, a unique neural unit for scans, etc. These neural units aim to learn sufficiently complex functions to model the performance of relational operators in a variety of contexts. For example, while a simple polynomial model of a join operator may make predictions only based on estimated input cardinalities, our neural units will automatically  identify the most relevant features out of a wide number of candidate features (i.e., underlying structure of the table, statistics about the data distribution, uncertainty in selectivity estimates, available buffer space, etc.), all without any hand-tuning.


\begin{figure}
\centering
\includegraphics[width=0.38\textwidth]{figures/scan_unit-crop.pdf}
\caption{\small Neural unit corrosponding to a relational scan operator,~$N_{s}(\frown)$. The neural unit take input from no children (it corrosponds to a leaf). }
\label{fig:scan_unit}
\end{figure}


Figure~\ref{fig:scan_unit} shows an example of one such neural unit for a table scan operator. The unit takes information from the query plan (e.g., index/table scan, optimizer’s predicted cost, cardinality estimates,  estimated I/Os, memory availability, etc). These inputs are fed through a number of hidden layers. Then, the output layer transforms the internal representation learned by the hidden layers into a latency prediction. On its own, each neural unit is expected to  predict the performance of an individual operator; for example, neural units corresponding to joins would predict the latency of a join operator.


\sparagraph{Formalizing neural units} We next describe the neural units formally, before proceedings with two examples. We first define the feature vector of a relational operator instance $x$ as $F(x)$. Note that the size of the output of $F(x)$ may vary based on the type of $x$: following Figure~\ref{fig:features}, if $x$ is a join operator, $F(x)$ could produce a vector of size 9, whereas if $x$ is a scan operator, $F(x)$ could produce a vector of size 7. We assume that $F(x)$ produces the same size vector for every \emph{instance} of a relational operator of fixed type, e.g. all scan operators have the same size feature vector. $F(x)$ could be implemented in many ways, such as executing an \texttt{EXPLAIN} query to get the optimizer's internal cost predictions, join type selection, etc. 

Next, we define a \emph{neural unit} as a neural network $N_A$, with $A$ representing the type of relational operator, e.g. $N_{\bowtie}$ is the neural unit for a join operator. Each neural unit $N_A$ contains a set of weights and biases (see Section~\ref{sec:nn}), and each neural unit produces an output vector $\vec{v}$ of size $d + 1$. The first element of $\vec{v}$ represents the neural unit's estimation of the operator's latency, labeled $N_A(x)_l$, and the other elements represent a size $d$ opaque representation of the operator passed on to the parent neural unit, labeled $N_A(x)_d$.
% These values correspond to the $R_l$ and $R_f$ values of recurrent neural networks, as discussed in Section~\ref{sec:rnn}.
To compute these values, each neural unit takes as input the feature vector generated by $F$, in addition to the $N_A(y)$ output of $x$'s children. Letting the children of $x$ be $x_0, x_1, \dots, x_i$, and letting the relational operator type of each of $x$'s children be $B, C, \dots, Z$:

\begin{equation}
\label{eq:neural_unit}
N_A\left( F(x) \frown N_B(x_0) \frown ... \frown N_Z(x_i) \right) = \vec{v}
\end{equation}

Above, each $\frown$ symbol represents the vector concatenation operator. When a relational operator has no children (such as a scan), $N_A$ can be written simply as $N_A(x) = n_A(F(x))$. Because each operator has different features, the inputs to the different neural units will not be the same shape: for example, following Figure~\ref{fig:features}, the feature vector produced by  $F$ for a scan operation may be a vector of length 7, but the feature vector produced by $F$ for a join operation may be a vector of length 9. Because of this, each neural unit may have a different sizes of weight and bias vectors.



\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figures/nn_details-crop.pdf}
\caption{\small Neural unit corrosponding to a relational join operator,~$N_{\bowtie}(\frown)$. The neural unit takes input from two children and several optimizer features.}
\label{fig:nn_detail}
\end{figure}

\sparagraph{Example: joins} Figure~\ref{fig:nn_detail} shows an example of one such neural unit, corresponding to a join operator ($N_{\bowtie}$). The unit takes information from its children, represented by two data outputs and one latency prediction, as well as information about the join operator itself (the type of join, the optimizer's predicted cost, cardinality estimates, etc.). These inputs are fed through a number of hidden layers. Finally, the internal representation learned by the hidden layer is transformed into two data outputs ($N_{\bowtie}(\frown)_d$) and a latency prediction ($N_{\bowtie}(\frown)_l$). The data outputs are some opaque representation of the join operator that is passed on to the parent neural unit (if any), just like the $R_f$ component of a traditional recurrent neural network. The latency outputs are trained to predict the latency of the join operator, just like the $R_l$ component of a traditional recurrent neural network. 

\sparagraph{Example: scans} Figure~\ref{fig:scan_unit} shows an example of a neural unit corresponding to a scan operator. Like the neural unit for the join operator, the neural unit for the scan operator also has a data output and a latency output, again corresponding to the $R_f$ and $R_l$ components of a traditional recurrent neural network. However, unlike the join neural unit, the scan neural unit has no children (as it corresponds to a leaf node in any query execution plan). Additionally, the scan neural unit takes in a different set of features than the join neural unit. While the join neural unit had input features like ``join type,'' the scan neural unit has input features like ``scan type.'' Since each \emph{operator} has homogeneous features (e.g., each instance of a scan operator has the same optimizer features), creating one neural unit to model each operator enables us to fully take advantage of the information available at each tree node, even though the nodes of the \QEP tree are heterogeneous.


\subsection{Plan-level neural networks}
\label{sec:tree}
Having constructed neural units for each operator type that may appear in a \QEP, we next explain how those neural units can be composed into tree structures isomorphic to any particular \QEP. Figure~\ref{fig:nn_general} shows an example of a \QEP and the isomorphic tree-structured neural network. Intuitively, each operator in a \QEP is replaced with its corresponding neural unit, e.g.~join operators are replaced with $N_{\bowtie}$, and the output of each neural unit is fed into the parent. Formally, we predict the latency of a \QEP with a root operator $r$ of type $R$ by evaluating $N_R(r)_l$. Note that the recursive definition (Equation~\ref{eq:neural_unit}) of $N_R(r)$ will ``replace'' each relational operator with the required neural unit in a top-down fashion.

\todo{WHERE?} Since the same neural unit will be used for each instance of a particular operator, the new architecture will still benefit from a recurrent neural network's weight sharing. However, since distinct operators will \emph{not} share weights between them, our new architecture will be able to handle the heterogenous nature of the query execution plan's tree nodes.



\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figures/tree_full-crop.pdf}
\caption{\small A neural network for a simple join query}
\label{fig:nn_full}
\end{figure}

An example of this construction is shown in Figure~\ref{fig:nn_full}. For the \QEP shown in the bottom right hand side of the figure (two table scans and a join), two instances of the scan neural unit and one instance of the join neural unit are created. The outputs of the scan units are concatenated together with the features of the join operator to make the input for the join unit, which produces the final latency prediction.

\begin{figure}
\centering
\includegraphics[width=0.38\textwidth]{figures/nn_overview-crop.pdf}
\caption{\small Neural network for QPP}
\label{fig:nn_overview}
\end{figure}

Figure~\ref{fig:nn_overview} shows a more general example, with a query plan (top left) and the corresponding neural network tree (right). Each neural unit, represented as trapezoids, takes in a number of inputs. For the leaf units (orange, corresponding to the table scans in the query plan), the inputs are features from the query plan (black arrows). The internal, non-leaf units take features from the query plan as well, but additionally take in the latency output (green arrows) and the data outputs (red arrows) of their children. The latency outputs represent the model’s estimate of the latency of each operator, and the data outputs contain information about each operator that may be useful to the parent operator (for example, the table scan neural unit may encode data about which relation is being read).  Here, the two orange trapezoids correspond to the table scan operators of $R_1$ and $R_2$ in the query plan, and thus share the same set of weights.

Next, we explain how this tree-structured neural network architecture solves the issues outlined in Section~\ref{sec:issues}.

\begin{itemize}
\item{{\bf Branch isolation}: Since we know that any particular relational operator in a \QEP can only affect the performance of its ancestors, and not its siblings or children, we say that a \QEP exhibits branch isolation. The way we assemble neural units into trees respects this property: each neural unit passes information exclusively upwards. Intuitively, this upwards-only communication policy directly encodes  knowledge about the structure of the query execution plan (branch isolation) into the network architecture itself.}
%\item{{\bf Single output}: Critically, each neural unit (corresponding to a type of relational operator) takes different shapes of input (depending on the features of the operator), but \emph{produces the same output shape,} allowing the children of a particular neural unit to be of arbitrary type (e.g., the children of a join operator may be another join, a table scan, a filter, etc.). The output of the root node can be used as a single value for predicting the latency of the entire tree.}
\item{{\bf Heterogeneous tree nodes}: By structuring each neural unit to take in a specific number of inputs corresponding to the features available, but produce the same number of outputs, arbitrary tree structures can be assembled.}
\end{itemize}



%The entire query plan is modeled as trees of neural units. For example, consider the simple query plan in the lower-right hand corner of Figure~\ref{fig:nn_full}. Two scan operators are fed into a join operation. The rest of Figure~\ref{fig:nn_full} shows an example of how the neural unit for the ``scan'' operator and the neural unit for the ``join'' operator can be combined. Since operators share some similar characteristics regardless of their position in the query plan, the internal weights of the neural unit corresponding to each operator type (e.g. scan) are shared, so that a single set of weights predicts the latency of any instance of an operator.




\section{Model training}\label{sec:model-training}

So far, we have discussed how to assemble neural units into trees matching those of a \QEP. However, each neural unit (specifically, the weights and biases they contain)  will require training. Like any neural network, the neural units are trained using gradient descent, as described in Section~\ref{sec:nn}.


The network is trained using a large corpus of executed query plans. For each subtree of the query plan (including the entire query plan), we construct a corresponding tree of neural units. Then, we measure the difference between what each subtree of neural units is predicting and the observed latency (the loss), and adjust the weights of each neural unit accordingly~\cite{Ruderoverviewgradientdescent2016}.  Over time, each neural unit learns to (1) predict the latency of itself and its subtree, and (2) provide useful output data for its parent neural unit. Note that we do not require the data outputs of any of the neural units to be a particular value -- the training algorithm is free to adjust these freely.

Formally, for a dataset of query operators $op \in D$, each with known latency $l(op)$ and operator type $t(op)$, the loss function we wish to minimize is:

\begin{equation}
\label{eq:loss}
L_2(D) = \sqrt{\frac{1}{|D|} \sum_{op \in D} \left(N_{t(op)}(op) - l(op)\right)^2}
\end{equation}

Since every component of $N_A$ is differentiable, and $L_2(D)$ is itself differentiable, Equation~\ref{eq:loss} can be effectively minimized using stochastic gradient descent~\cite{Ruderoverviewgradientdescent2016}. We next propose two improvements over naive methods for computing Equation~\ref{eq:loss} in the context of gradient descent.

\subsection{Shared information in subtrees}
One can save a significant amount of time when computing the loss function for multiple nodes in the same tree. Suppose that $r$ is a root of a \QEP, and $c$ is the sole child of that root. When computing the term $(N_{t(r)}(r) - l(r))^2$ in the summation in Equation~\ref{eq:loss}, we must compute $N_{t(c)}(c)$ as a intermediate value. This follows from the definition of $N_{t(r)}(r)$ in Equation~\ref{eq:neural_unit}:
\begin{equation*}
N_{t(r)}(r) = n_{t(r)}\left( F(r) \frown N_{t(c)}(c) \right)
\end{equation*}

Since $L_2(D)$ will \emph{also} require computing $(N_{t(c)}(c) - l(c))^2$, we can avoid a significant redundant computation by caching the value of $N_{t(c)}(c)$ so that it only needs to be computed once. More generally, for an arbitrary root $r \in D$, we can thus compute the error of each neural unit in the tree rooted at $r$ in a bottom-up fashion: first, for each leaf node $leaf$ in the tree rooted at $r$, compute and store the output the neural units corresponding to the leaf nodes: $N_{t(leaf)}(leaf)$. Then, compute and sum the $(N_{t(leaf)}(leaf) - l(leaf))^2$ values, storing the result into a global accumulator variable. Once all the leaf nodes have been resolved in this way, repeat the process moving one level up the tree. When the root of the tree has been reached, the global accumulator value will contain the $(N_A(x) - l(x))^2$ values for every node in the tree rooted at $r$.

\begin{figure}
\centering
\includegraphics[width=0.38\textwidth]{figures/tree_opt-crop.pdf}
\caption{\small Efficiently computing the sum of losses for each neural unit in a tree. The ``$-^2$'' nodes represent computing the difference and then squaring the result.}
\label{fig:tree_opt}
\end{figure}

\sparagraph{Example} Figure~\ref{fig:tree_opt} shows a graphical representation of this process. First, we compute and cache the output of the neural unit labeled ``1''. We then add the squared difference between the outputted latency and the true latency, $l(1)$ into the global accumulator variable $g$. Next, we compute and cache the output of the neural unit labeled ``2''. Note that to compute the output of ``2'', we reuse the cached output value of ``1''. Then, we compute the squared difference between the latency predicted by ``2'' and $l(2)$, adding the result into the global accumulator. The same process is repeated for neural unit ``3'', which has no children. Finally, we compute the output of neural unit ``4'', which requires reusing the cached outputs from neural units ``2'' and ``3''. We then compute the squared difference between the latency predicted by neural unit ``4'' and $l(4)$, and add it to the global accumulator variable.

The global accumulator $g$ now contains the sum of the squared differences between the predicted latency and the actual latency for every node in the tree. Applying this technique over every tree in $D$ can greatly accelerate the computation of the loss function (Equation~\ref{eq:loss}).


\subsection{Batch training}

% all data: too expensive. one at a time: too slow. mini-batch: not our technique, assumption doesn't match
% here's how we make mini-batch better
Training a neural network is generally a very expensive operation, since each neural unit could contain hundreds of thousands or even millions of weights. To tackle this challenge, modern differentiable programming frameworks like Tensorflow~\cite{tensorflow} and PyTorch~\cite{pytorch} preform training in \emph{batches}. Instead of computing the gradient using the entire dataset (which cannot effectively fit into memory), simple random samples (called batches or mini-batches) are drawn from the data and used to estimate the gradient. 

This approach works very well for neural networks where the structure of the network does not change based on the inputs (which is the case in most applications, e.g. computer vision and natural language processing), because the (symbolic) derivative of each weight will be identical for each item in the batch and their computation can thus be vectorized. However, this optimization poses a challenge for the proposed tree-structured model: if two samples in a batch have different tree structures, the (symbolic) derivative for a given weight will be different.

One solution might be to group the training set into query execution plans with identical structure, and then use each group as a batch. While this would be efficient, most of the effectiveness of batching depends on the batch being a true simple random sample. By only creating batches with identical tree structures, each batch, and thus each estimation of the gradient, will become biased.

Instead, we proposes constructing very large batches of randomly sampled query plans. Within each large batch, we group together query plans with identical structure. The gradient of each weight for each operator is then efficiently estimated within each inner-batch group, and the results are added together and normalized based on group size, ensuring the estimate of the gradient is not biased. For example, if a randomly-sampled large batch contained three groups, $B = \{G_1, G_2, G_3\}$ query executionplans with 10, 20, and 300 members each, the gradient of each weight would be estimated as follows:

\begin{align*}
  &\nabla_w (L_2(B)) = \frac{1}{10+20+300} \times \\
  &\bigg( 10 \frac{\partial L_2(G_1)}{\partial w} + 20 \frac{\partial L_2(G_2)}{\partial w} + 300 \frac{\partial L_2(G_3)}{\partial w}\bigg)\\
\end{align*}

This approach avoids biasing the gradient estimate while still gaining efficiency from batch processing. However, this optimization  comes at the cost of greater memory requirements.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "edbt2019"
%%% End:


==> rnns.tex <==
\subsection{Recurrent neural networks}
\label{sec:rnn}
While the neural networks described above have received significant attention, they map fixed-sized inputs to a fixed-size output: for example, a DNN might map vectors of size $30$ to an output of size $1$. However, query execution plans do not have a fixed size. The type of neural network used in this paper is a specialized version of a \emph{recurrent neural network}~\cite{pollack_ram,lstm,tree_lstm}. Recurrent neural networks (RNNs) generally operate on \emph{sequences} of fixed-size input vectors. RNNs produce an output for each input vector in the sequence, and this output depends on both the corresponding input vector \emph{and} the preceding input vectors. %Recurrent neural networks \change{are \emph{context sensitive}, meaning that the order in which input vectors are given to the network can change the network's output.}
This allows future decisions to be impacted by past observations. For a more detailed overview of RNNs, see~\cite{DeMuldersurveyapplicationrecurrent2015}.

\begin{figure}
\centering
\includegraphics[width=0.45\textwidth]{figures/rnn-crop.pdf}
\caption{\small Recurrent neural network}
\label{fig:rnn}
\end{figure}

At their core, an RNN consists of a single neural unit (a small neural network), which is ``unrolled'' or ``tiled'' $n$ times, where $n$ is the length of the input sequence (illustrated in Figure~\ref{fig:rnn}). The neural unit takes in two values -- one value from the previous neural unit, and one value from the input sequence. Each neural unit of an RNN also produces two values -- a label, and a value that is passed to the next recurrent unit. For example, Figure~\ref{fig:rnn} shows a simple recurrent neural network labeling the parts-of-speech of each word in the input sequence. The word ``The'' is fed into the first neural unit, and the neural unit produces (1) an output representing the label ``A'', for ``article'', and (2) an output that is passed to the next neural unit. The next neural unit receives (1) the output of the previous unit, and (2) the next item from the input sequence (``quick'').

Critically, each neural unit in a recurrent neural network \emph{share the same weights.} When the network is unrolled or tiled, the weights of all neural units (four in the example figure) share the exact same weights. Letting the label produced by a neural unit be $R_l(p, s)$ and letting the data passed to the next neural unit be  $R_f(p, s)$, where $p$ represents the previous value and $s$ represents corresponding vector from the input sequence, the output ``N'' in the figure above is:

\begin{equation*}
R_l(R_f(R_f(R_f(\vec{0}, \mbox{``The''}), \mbox{``quick''}), \mbox{``brown''}), \mbox{``fox''}) = \mbox{``N''}
\end{equation*}

The value passed to the next recurrent unit, $R_f(p, s)$, is often described as ``opaque'' or ``encoded,'' because it is a purely \emph{learned} value that might not directly match up with the input data -- it is a representation of the previous sequence members that the recurrent neural network has learned. For example, this learned value might somehow encode that the previous word was an adjective, which might increase the probability that the next word is a noun. However, it is important to note that the designer need not -- and generally, cannot -- specify what sort of information this passed value contains. The recurrent neural network will \emph{automatically} learn what sort of information needs to be passed to the next unit, and how to encode it. It does so through the training process: each iteration of gradient descent tweaks the values of the weights controlling how the passed value is computed.


It is important to remember that, like Equation~\ref{eq:nn}, both $R_l(p, s)$ and $R_f(p, s)$ are compositions of differentiable functions, and are thus themselves differentiable. When many example input sequences and output labels are provided, we can define a loss function similar to Equation~\ref{eq:ex_loss}. For example, given a single sequence of size 3, $s$, and the three corresponding labels $b$, we can write the loss function for the sequence as:

\begin{equation*}
\begin{split}
  serr(s, b, R) &= (R_l(\vec{0}, s_1) - b_1)^2\\
  & + (R_l(R_f(\vec{0}, s_1), s_2) - b_2)^2 \\
  & + (R_l(R_f(R_f(\vec{0}, s_1), s_2), s_3) - b_3)^2
\end{split}
\end{equation*}

Given a set of input sequences $S$ and sequence labels $B$, we can write the loss function for the whole recurrent neural network as:
\begin{equation*}
rerr(S, B, R) = \sqrt{\frac{1}{|S|} \sum_{s, b \in S, B} \frac{serr(s, b, R)}{|s|} }
\end{equation*}


Like before, $rerr$ can be differentiated with respect to each weight, e.g. the gradient can be computed as previously described, and gradient descent methods can be applied. The critical insight to take away from this is that, while the loss function is clearly minimized when the output labels, $R_l$, are correct, \emph{there is absolutely no restriction on what the value passed to the next unit, $R_f$ can produce}. The RNN is thus ``free'' to use $R_f$ however it chooses, and gradient descent (given our loss function), will push the RNN to choose the weights controlling $R_f$ in such a way that makes $R_l$ easier to compute. This happens \emph{automatically}. In the next section, we will use a similar approach to help neural units learn interactions between physical operators in a DBMS. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "edbt2019"
%%% End:

